Application of Herglotz's Variational Principle to Electromagnetic Systems with Dissipation

This work applies the contact formalism of classical mechanics and classical field theory, introduced by Herglotz and later developed in the context of contact geometry, to describe electromagnetic systems with dissipation. In particular, we study an electron in a non-perfect conductor and a variation of the cyclotron radiation. In order to apply the contact formalism to a system governed by the Lorentz force, it is necessary to generalize the classical electromagnetic gauge and add a term in the Lagrangian. We also apply the k-contact theory for classical fields to model the behaviour of electromagnetic fields themselves under external damping. In particular, we show how the theory describes the evolution of electromagnetic fields in media under some circumstances. The corresponding Poynting theorem is derived. We discuss its applicability to the Lorentz dipole model and to a highly resistive dielectric.

==> Comandos.tex <==

\newcommand{\fline}{\overline{f}}
\newcommand{\gline}{\overline{g}}

\newcommand{\R}{\mathbb{R}}
\newcommand{\D}{\mathbb{D}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\K}{\mathbb{K}}
\renewcommand{\S}{\mathbb{S}}
\newcommand{\T}{\mathbb{T}}

\newcommand{\id}{\mathrm{id}}

\newcommand{\SO}{\operatorname{SO}}

\newcommand{\lap}{\bigtriangleup}

==> Preambulo.tex <==
\usepackage[catalan]{babel}
\usepackage[utf8]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{graphics,graphicx}
\usepackage{xcolor}
\usepackage{wasysym}
\usepackage{tikz}
\usepackage{amsthm}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{mathtools}
\usepackage{mathrsfs}
\usepackage{amsfonts}
\usepackage{float}
\usepackage{enumerate}
\usepackage{tikz-cd}
\usetikzlibrary{babel}
\usepackage{caption}
\usepackage{subfigure}
\usepackage{comment}
\usepackage{ esint }
\usepackage{tikz-cd}
\usepackage{tikz}
\usetikzlibrary{arrows,shapes,cd}
%\setbeamercolor{math text}{black}

\theoremstyle{definition}
\newtheorem{defi}{Definition}
\newtheorem{eje}{Example}
\theoremstyle{plain}
\newtheorem{teo}{Theorem}
\newtheorem{obs}{Remark}
\newtheorem{coro}{Corollary}
\newtheorem{prop}{Proposition}
\newtheorem{lem}{Lemma}


\setbeamertemplate{footline}
{
	\leavevmode%
	\hbox{%
		\begin{beamercolorbox}[wd=.18\paperwidth,ht=2.25ex,dp=1ex,center]{author in head/foot}%
			\usebeamerfont{author in head/foot}\insertshortauthor
		\end{beamercolorbox}%
		\begin{beamercolorbox}[wd=.82\paperwidth,ht=2.25ex,dp=1ex,center]{title in head/foot}%
			\usebeamerfont{title in head/foot}\insertshorttitle\hspace*{.5em}
			\insertframenumber{} / \inserttotalframenumber\hspace*{.5ex}
	\end{beamercolorbox}}%
	\vskip0pt%
}

\title[Application of Herglotz's Variational Principle to Electromagnetic Systems with Dissipation]{ Application of Herglotz's Variational Principle \\ to Electromagnetic Systems with Dissipation}
\author[A. Marín, J. Gaset]{Adrià Marín\inst{1} and Jordi Gaset\inst{2}}
\institute[]{
	\inst{1}
	Department of Mathematics, Department of Physics\\
	Universitat Autònoma de Barcelona
	\and
	\inst{2}
	Department of Physics\\
	Universitat Autònoma de Barcelona
}
\date[]{XXIX International Fall Workshop in Geometry and Physics\\September 2021}
